Feature Distribution on Graph Topology Mediates the Effect of Graph Convolution: Homophily Perspective

How would randomly shuffling feature vectors among nodes from the same class affect graph neural networks (GNNs)? The feature shuffle, intuitively, perturbs the dependence between graph topology and features (A-X dependence) for GNNs to learn from. Surprisingly, we observe a consistent and significant improvement in GNN performance following the feature shuffle. Having overlooked the impact of A-X dependence on GNNs, the prior literature does not provide a satisfactory understanding of the phenomenon. Thus, we raise two research questions. First, how should A-X dependence be measured, while controlling for potential confounds? Second, how does A-X dependence affect GNNs? In response, we (i) propose a principled measure for A-X dependence, (ii) design a random graph model that controls A-X dependence, (iii) establish a theory on how A-X dependence relates to graph convolution, and (iv) present empirical analysis on real-world graphs that align with the theory. We conclude that A-X dependence mediates the effect of graph convolution, such that smaller dependence improves GNN-based node classification.

==> results/algorithm/csbmx.tex <==
\begin{algorithm}[t]
    % \small
   \caption{\text{\gmodel}}\label{algo:csbmx}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} 
    number of nodes $n$, 
    % class probability $q$, 
    feature mean vector $\mu_{\ell}$'s and covariance matrix $\Sigma_\ell$'s, 
    same- and different-class degree $d^+$ and $d^-$, 
    and \ax strength $\tau$.
    

    % \STATE {\bfseries Output:} \gmodel Graph 
    \vspace{1.8mm}

    \blue{${/}^{*}$ Step 0. Initialize nodes, edges, and class ${}^{*}/$} \\
    \STATE $V \leftarrow [n], ~E \leftarrow \emptyset$
    \vspace{0.7mm}
    \STATE {$Y \leftarrow \text{~a random permutation of~}     
    [\mathbf{0}_{\frac{n}{2}} \Vert \mathbf{1}_{\frac{n}{2}}]$}
    % , where $\mathbf{0}, \mathbf{1} \in \mathbb{R}^{\frac{n}{2}}$}
    
    \vspace{1.8mm}
    \blue{${/}^{*}$ Step 1. Sample node features ${}^{*}/$} \\
    \FOR{$v_i \in V$}
        % \STATE $Y_i \sim \bernoulli(p)$ \footnotemark
        % \STATE $Y_i \sim \operatorname{Bernoulli}(0.5)$
        \vspace{0.7mm}
        \STATE $X_i \sim \calN(\mu_{Y_i},~\Sigma_{Y_i})$
        \vspace{0.7mm}
    \ENDFOR

    \vspace{1.8mm}
    \blue{${/}^{*}$ Step 2. Sample directed edges ${}^{*}/$} \\


    \FOR{$v_i \in V$}
    
        \vspace{0.7mm}
        % \STATE $\phi_{ij} = \exp(\tau \cdot \mathbf{h}^{(p)}_{ij}),\forall v_j \in V'_i$ 

        \STATE $\mathbf{C}^{+}_{i} \leftarrow [j]_{v_{j} \in {C}^{+}_{Y_{i}} \setminus \{v_{i}\}}$ , 
        $\mathbf{\Phi}^+_i \leftarrow [e^{\tau \mathbf{h}^{(p)}_{ij}} : j = \mathbf{C}^{+}_{i,t}]_{t=1}^{\vert {C}^{+}_{Y_{i}}\vert - 1}$

        \STATE $\mathbf{C}^{-}_{i} \leftarrow [j]_{v_{j} \in {C}^{-}_{Y_{i}}}\quad~~~$ , 
        $\mathbf{\Phi}^-_i \leftarrow [e^{\tau \mathbf{h}^{(p)}_{ij}} : j = \mathbf{C}^{-}_{i,t}]_{t=1}^{\vert {C}^{-}_{Y_{i}}\vert}$

        %\STATE $\mathbf{\Phi}^+_i \leftarrow [\exp(\tau \cdot \mathbf{h}^{(p)}_{ij})]_{\forall v_j \in {C}^{+}_{Y_{i}} \setminus \{v_{i}\}}$
        %\STATE $\mathbf{\Phi}^-_i \leftarrow [\exp(\tau \cdot \mathbf{h}^{(p)}_{ij})]_{\forall v_j \in {C}^{-}_{Y_{i}}}$
        
        \vspace{0.7mm}
        \STATE $ N^{+}_{i} \leftarrow {\operatorname{WS_{wr}}} (\mathbf{C}^{+}_{i},~ \mathbf{\Phi}^+_i,~ d^+)$ 
        ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \footnotesize (\blue{$\ast$}) \normalsize 
        
        \vspace{0.7mm}
        \STATE $ N^{-}_{i} \leftarrow {\operatorname{WS_{wr}}}  (\mathbf{C}^{-}_{i},~ \mathbf{\Phi}^-_i,~ d^-)$

        \vspace{0.7mm}
        \STATE $ E \leftarrow E \cup \set{(v_i, v_j)}, \forall v_{j} \in (N^{+}_{i} \cup N^{-}_{i}$)~~\footnotemark
        \vspace{0.7mm}
        % \FOR{$v_{j} \in V^{+}_{i} \cup V^{-}_{i}$}
        %     \STATE $ E = E \cup \set{(v_i, v_j)}$\footnotemark
        % \ENDFOR
        % \footnotesize (\blue{$\ast \ast$}) \normalsize  
    \ENDFOR
    \vspace{1.8mm}
    
    \STATE \textbf{return} $\mathcal{G} \coloneqq \mathcal{G}(n, \mu_\ell, \Sigma_\ell, d^+, d^-, \tau) = (V, E)$ 
    ~~~~~~~~~~~~~ \footnotesize (\blue{$\ast \ast$})
    \vspace{0.1mm}
    
    \footnotesize
    (\blue{$\ast$}) $\operatorname{WS_{wr}}({\mathbf{C}}, \mathbf{\Phi}, d)$ denotes weighted sampling without replacement given 
    a vector of population ${\mathbf{C}}$, 
    a sample weight vector $\mathbf{\Phi}$, 
    and the sample size $d$.    

    \vspace{0.7mm}
    (\blue{$\ast \ast$}) Each node $v_i \in V$ has class $Y_i$ and features $X_i$.
    \vspace{0.7mm}

\end{algorithmic}
\end{algorithm}

% \footnotetext{In \gmodel, $(v_i, v_j)$ denotes a directed edge from $v_i$ to $v_j$.}


==> results/figs/measure_intuition.tex <==
\begin{figure}[t] 
    \centering
    \vspace{2mm}
    
    \includegraphics[width=\linewidth]{results/raw_data/sec3_intuition.pdf}

    \caption{\label{fig:measure_intuition}
    \bolden{A Visual Intuition of CFH \hdot.}
    Note that (\textit{i}) WK $(X)$ is no longer homophilic after controlling for AG $(Y)$
    and (\textit{ii}) homophily, heterophily, and random are determined relative to homophily baseline $b(\cdot)$.
     }
    \vspace{2mm}
\end{figure}

